Data-Agnostic Face Image Synthesis Detection Using Bayesian CNNs

Face image synthesis detection is considerably gaining attention because of the potential negative impact on society that this type of synthetic data brings. In this paper, we propose a data-agnostic solution to detect the face image synthesis process. Specifically, our solution is based on an anomaly detection framework that requires only real data to learn the inference process. It is therefore data-agnostic in the sense that it requires no synthetic face images. The solution uses the posterior probability with respect to the reference data to determine if new samples are synthetic or not. Our evaluation results using different synthesizers show that our solution is very competitive against the state-of-the-art, which requires synthetic data for training.

==> DATA/FIGS/FIG_Parms.tex <==
\begin{figure}[h]
\begin{center}
\includegraphics[width=0.5\textwidth]{./DATA/FIGS/FIG_Parms.pdf}
\caption{ \small{ The model's posterior for different number of parameters with and without dropout in the \acrshort{FC} layers  }  }
\label{fig:parms}
\end{center}
\end{figure}


==> DATA/authors.tex <==
\author[label1]{Roberto Leyva\corref{orcid}}
\ead{marcial.leyva-fernandez@warwick.ac.uk}
\author[label2]{Victor Sanchez}
\ead{v.f.sanchez-silva@warwick.ac.uk}
\author[label1]{Gregory Epiphaniou}
\ead{gregory.epiphaniou@warwick.ac.uk}
\author[label1]{Carsten Maple}
\ead{cm@warwick.ac.uk}


\address[label1]{WMG, University of Warwick, CV47AL, Coventry, UK}
\address[label2]{Department of Computer Science, University of Warwick, CV47AL, Coventry, UK}


%\author[1]{Roberto Leyva\corref{cor1}\fnref{orcid}}

\fntext[orcid]{Corresponding author, orcid=0000-0003-4561-8798, R. Leyva is also with ITESM, corresponding email: rleyv@tec.mx. This work is partly funded by the Alan Turing Institute via Bill \& Melinda Gates Foundation.}
%\fntext[note2]{R. Leyva is also with ITESM Campus Toluca, contact rleyv@tec.mx}
%\cortext[cor1]{Corresponding author}


%\author[2]{Victor Sanchez}

%\author[1]{Gregory Epiphaniou}

%\author[1]{Carsten Maple}


           
%\affiliation[1]{organization={WMG, University of Warwick},
%            addressline={CV47AL}, 
%            city={Coventry},
%            country={UK}}

%\affiliation[2]{organization={Department of Computer Science, University of Warwick},
%            addressline={CV47AL}, 
%            city={Coventry},
%            country={UK}}
            


==> DATA/config.tex <==
%\usepackage[compress,numbers]{natbib}
%\usepackage[authoryear,longnamesfirst]{natbib}
\biboptions{longnamesfirst,numbers,compress}

\usepackage{overpic}
\usepackage{xcolor}
\usepackage{xurl}
\usepackage{multirow}
\usepackage{soul}
\usepackage{subcaption}
\usepackage{float}
\usepackage[acronym]{glossaries}

\makeglossaries
\loadglsentries{./DATA/gls.tex}
\glsenablehyper

\usepackage{booktabs}

\usepackage[colorlinks]{hyperref}

\captionsetup[figure]{labelfont={bf},name={Fig.},labelsep=period}

\usepackage{wrapfig}
\usepackage{graphicx}

\usepackage{arydshln}
